REAPER: Reasoning based Retrieval Planning for Complex RAG Systems

Complex dialog systems often use retrieved evidence to facilitate factual responses. Such RAG (Retrieval Augmented Generation) systems retrieve from massive heterogeneous data stores that are usually architected as multiple indexes or APIs instead of a single monolithic source. For a given query, relevant evidence needs to be retrieved from one or a small subset of possible retrieval sources. Complex queries can even require multi-step retrieval. For example, a conversational agent on a retail site answering customer questions about past orders will need to retrieve the appropriate customer order first and then the evidence relevant to the customer's question in the context of the ordered product. Most RAG Agents handle such Chain-of-Thought (CoT) tasks by interleaving reasoning and retrieval steps. However, each reasoning step directly adds to the latency of the system. For large models this latency cost is significant -- in the order of multiple seconds. Multi-agent systems may classify the query to a single Agent associated with a retrieval source, though this means that a (small) classification model dictates the performance of a large language model. In this work we present REAPER (REAsoning-based PlannER) - an LLM based planner to generate retrieval plans in conversational systems. We show significant gains in latency over Agent-based systems and are able to scale easily to new and unseen use cases as compared to classification-based planning. Though our method can be applied to any RAG system, we show our results in the context of a conversational shopping assistant.

==> _old/07-27-2024/evaluation.tex <==
\section{Experiments}

In this section we present experimental setting and results  comparing REAPER against \ift, Claude3-Sonnet and the our ensemble classifier described in Section~\ref{sec:curr-system}. Our experiments show the need for fine-tuning for the plan generation as larger models like Claude3-Sonnet or Mistral tend to hallucinate. We also present ablation studies to show the impact of different components that we proposed to create our training data. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Claude_Plan_Generation_1.png}
    % \caption{Example: Claude plans }
    %\label{fig:claude-plans-2}
%\end{figure}
% \end{wrapfigure}

% \begin{wrapfigure}{r}{0.66\textwidth}
%\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Claude_Multi_Step_Plan_Generation_2.png}
    \caption{Example Claude3-Sonnet plans. Similar to Mistral, we also see hallucinations in plans. For example, extra step in the second plan and extra explanation in the third plan. With more effort it may be possible to reduce hallucinations. Claude3-Sonnet latency though, is 10x of Mistral latency.}
    \label{fig:claude-plans-2}
\end{figure}

\subsection{Comparison with Open Models}
%\aj{@Sheikh, @Shrivats please go over this and confirm/change}
%We spent several weeks prompt tuning the the ift  model to generate REAPER response using in-context learning. However, we were unable to get the model to not hallucinate tools or plans. 
It is generally desirable to solve a task using a language model using in-context learning. Despite our several weeks worth of effort, we could not prompt-tune \ift to reach the target performance. Figure~\ref{fig:mistral-plans-1} shows examples of the plans generated by \ift with prompt tuning. We also tested out our REAPER prompt on Claude3-Sonnet (Figure~\ref{fig:claude-plans-2}) and could not prevent hallucinations. In addition, Claude3-Sonnet latency was $\sim2$s per step as compared to 207ms for the entire plan for REAPER and Mistral models -- introducing an order of magnitude latency cost in addition to more powerful hardware required to run Claude3-Sonnet. 

\begin{table*}[tb]
    
\caption{Comparison of REAPER performance with Baselines on six retrieval classes}
\label{tab:overall_performance}
\begin{tabular}{|c|lll|llll|llll|}
\hline
                               & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}l@{}}Mistral\\ (No fine-tuning)\end{tabular}} & \multicolumn{4}{c|}{Ensemble Classifier}                                                                                                   & \multicolumn{4}{c|}{REAPER}                                                                                                                   \\ \hline
Classes                        & \multicolumn{1}{l|}{P}             & \multicolumn{1}{l|}{R}             & F1            & \multicolumn{1}{l|}{P}  & \multicolumn{1}{l|}{R}   & \multicolumn{1}{l|}{F1} & \begin{tabular}[c]{@{}l@{}}\#Training\\ Examples\end{tabular} & \multicolumn{1}{l|}{P}   & \multicolumn{1}{l|}{R}   & \multicolumn{1}{l|}{F1} & \begin{tabular}[c]{@{}l@{}}\#Training\\ Examples\end{tabular} \\ \hline
Customer Support                     & \multicolumn{1}{l|}{90}            & \multicolumn{1}{l|}{61}            & 73            & \multicolumn{1}{l|}{95} & \multicolumn{1}{l|}{81}  & \multicolumn{1}{l|}{88} & \multicolumn{1}{c|}{24621}                                                              & \multicolumn{1}{l|}{95}  & \multicolumn{1}{l|}{94}  & \multicolumn{1}{l|}{94} &   \multicolumn{1}{c|}{1127}                                   \\ \hline
Shipment Status                   & \multicolumn{1}{l|}{97}            & \multicolumn{1}{l|}{72}            & 83            & \multicolumn{1}{l|}{96} & \multicolumn{1}{l|}{96}  & \multicolumn{1}{l|}{96} & \multicolumn{1}{c|}{16150}                                                              & \multicolumn{1}{l|}{98}  & \multicolumn{1}{l|}{94}  & \multicolumn{1}{l|}{96} & \multicolumn{1}{c|}{996}                                                              \\ \hline
Product Search                 & \multicolumn{1}{l|}{82}            & \multicolumn{1}{l|}{65}            & 72            & \multicolumn{1}{l|}{84} & \multicolumn{1}{l|}{99} & \multicolumn{1}{l|}{91} & \multicolumn{1}{c|}{38683}                                                              & \multicolumn{1}{l|}{91}  & \multicolumn{1}{l|}{100} & \multicolumn{1}{l|}{95} & \multicolumn{1}{c|}{1289}                                                              \\ \hline
Product QnA & \multicolumn{1}{l|}{47}            & \multicolumn{1}{l|}{80}            & 59            & \multicolumn{1}{l|}{98} & \multicolumn{1}{l|}{97}  & \multicolumn{1}{l|}{98} &                 \multicolumn{1}{c|}{30813}                                              & \multicolumn{1}{l|}{93}  & \multicolumn{1}{l|}{99}  & \multicolumn{1}{l|}{96} & \multicolumn{1}{c|}{1045}                                                              \\ \hline
Review Summary                 & \multicolumn{1}{l|}{79}            & \multicolumn{1}{l|}{93}            & 85            & \multicolumn{1}{l|}{99} & \multicolumn{1}{l|}{96}  & \multicolumn{1}{l|}{97} & \multicolumn{1}{c|}{9875}                                                              & \multicolumn{1}{l|}{100} & \multicolumn{1}{l|}{94}  & \multicolumn{1}{l|}{97} & \multicolumn{1}{c|}{594}                                                              \\ \hline
No-retrieval             & \multicolumn{1}{l|}{85}            & \multicolumn{1}{l|}{67}            & 75            & \multicolumn{1}{l|}{98} & \multicolumn{1}{l|}{99}  & \multicolumn{1}{l|}{99} & \multicolumn{1}{c|}{35934}                                                              & \multicolumn{1}{l|}{100} & \multicolumn{1}{l|}{93}  & \multicolumn{1}{l|}{96} & \multicolumn{1}{c|}{1245}\\
\hline 
\hline
Tool Accuracy        & \multicolumn{3}{c|}{72\%}  & \multicolumn{4}{c|}{94\%}    & \multicolumn{4}{c|}{\textbf{96\%}} \\
\hline 
\hline
Argument Accuracy        & \multicolumn{3}{c|}{--}  & \multicolumn{4}{c|}{{88\%}}    & \multicolumn{4}{c|}{\textbf{92\%}}

% \\ \hline
% Human Small Talk               & \multicolumn{1}{l|}{91}            & \multicolumn{1}{l|}{72}            & 80            & \multicolumn{1}{l|}{-}  & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}  & \multicolumn{1}{c|}{-}                                                              & \multicolumn{1}{l|}{94}  & \multicolumn{1}{l|}{91}  & \multicolumn{1}{l|}{92} & \multicolumn{1}{c|}{286}     

\\ \hline
                               % & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}              &               & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   &                                                               & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   &                                                               \\ \hline
\end{tabular}
\end{table*}

\subsection{Comparison with Classifier-based Planners}

Our ensemble classifier is described in Section~\ref{sec:curr-system}. We evaluate the models along two dimensions:
\begin{enumerate}[leftmargin=0.1cm]
    \item \textbf{Tool Selection:} Given a query, we manually evaluate if the model selects the correct tool(s) in the proper sequence to retrieve evidence. As multi-step retrieval is just another class in the production system, this metric can be directly compared to the classification metrics of the production system.  We present accuracy, precision, recall and F1-score for this evaluation. 
    %On balanced evaluation set that includes queries requiring roughly equal proportion of the six tools available to REAPER, we manually evaluate the plans to ensure both that the right tools are selected and they are in the right sequence. This also allows us to compare against the production system of 2 Roberta classification models, that classifies queries into six classes. 
    \item \textbf{Argument Extraction:} The other aspect of REAPER is the accuracy of the arguments fed to the tools (refer Figure~\ref{fig:reaper-plans}). In the current setting, only two tools \texttt{prod\_search} and \texttt{shipment\_status} require the arguments different from the customer query. We thus restrict our evaluation to plans involving these tools. Our baseline system uses the \ift model to generate the arguments using a prompt specifically tuned for each class. REAPER does both tool selection and argument generation for all the tools in a single prompt. 
\end{enumerate}

\vspace{0.3cm}
Table~\ref{tab:overall_performance} shows the training data size and precision, recall and F1 metrics for REAPER, the baseline ensemble and \ift\ with only in-context tuning. Given Mistral tool accuracy is so low, we did not compute the Argument accuracy for it. %that model. 

\subsubsection{Evaluation Datasets}

Since Rufus is new, its traffic distribution is still skewed towards existing traffic patterns instead of the new use cases that Rufus intends to address. So instead of sampling traffic to generate our evaluation set, 
%we cannot sample traffic to create our evaluation set, since the distribution is skewed towards existing traffic patterns instead of the new use cases that Rufus intends to address. Instead 
we use a balanced evaluation set of 600 queries such that the corresponding plans have a roughly equal proportion of tools (classes) %, and 2) a traffic weighted evaluation set of 4778 queries, to ensure that we perform well on production traffic. Thus, we treat this dataset as a binary \texttt{prod\_search} and \texttt{not\_prod\_search} dataset and present precision, recall metrics on the binary classes. 

% \vspace{0.3cm}
% Table~\ref{tab:overall_performance} shows the training data size and precision, recall and F1 metrics for REAPER, the baseline ensemble and \ift\ with only in-context tuning. Given Mistral tool accuracy is so low, we did not compute the Argument accuracy for it. %that model. 



% \subsection{Baselines}

% We spent several weeks trying to get the Mistral-Instruct-v0.2 model to generate REAPER response using in-context learning. However, we were unable to get the model to not hallucinate tools or plans. Figure~\ref{fig:reaper-plans-mistral} shows examples of the plans generated by Mistral. \aj{Compare against Claude3-Sonnet}. We also test against the current production system, which consists of an ensemble of 2 Roberta models followed by a Mistral LLM which is used to extract keywords when necessary. 

% Finally, we want the model to have the following capabilities:
% \begin{enumerate}
%     \item \textbf{Adding a new tool:} Since Rufus will add several retrievers and tools to handle new use cases, we want to ensure that REAPER is able to easily onboard new tools. 
%     \item \textbf{Unseen use cases:} It is impossible to cover the entire conversational landscape in the training data. We want to ensure that REAPER is able to reason through new use cases. This means that REAPER should be able to generate a query plan using existing tools even though REAPER has never seen the plan before. 
% \end{enumerate}









% \section{REAPER}
% \aj{This has been discussed in section 4}
% Requirement for reasoning for a specific task. General reasoning ability not required 

% \subsection{LLM based planning}
% \aj{Move to the end in a Discussion/Analysis section}
% SFT vs IFT: Why not use code whisperer

% \subsubsection{Training data ablations}

% \section{Experiments}

% %The primary advantage of using an LLM for query execution planning is it solves a variety of query processing tasks text generation. When an LLM generates tools with parameters it performs both classification and information extraction. In this section we pro

% %We evaluate the LLMs ability to classify and extract based on the same datasets but using different evaluation metrics.  


% \subsection{Dataset}

% \textbf{Source Generation}: \
% This dataset assesses the retrieval accuracy of the model across diverse tool utilization scenarios within the context of customer queries. To ensure robustness in our evaluation across different retrieval scenarios, the dataset ensures a balanced representation of customer queries spanning various tool categories denoted as 'R', 'S', 'N', 'NO', 'P', and 'W'.

% Given that customer queries for 'R' and 'S' tools predominantly occur within the context of specific detail pages, we employed a two-stage process to simulate organic contexts facilitated by Claude3-Sonnet-Sonnet Sonnet language model. However, recognizing the potential for customers to also frame queries related to classes 'N', 'NO', 'P', and 'W' from detail pages, we introduced a mechanism to emulate such behavior by incorporating irrelevant contexts for 25\% of queries pertaining to these classes, while maintaining empty contexts for the remainder.

% The two-stage process begins with extracting relevant product-related keywords from the query prompt, followed by crafting highly specific product titles based on these extracted keywords. This method mitigates the inherent challenge of directly formulating organic and realistic product titles from customer queries by breaking down the task into manageable sub-steps, thereby ensuring the generation of contextually relevant data.


% \begin{table}[h]
% \centering
% \caption{Distribution of Source Generation Data Among Different Tools}
% \begin{tabular}{@{}cr@{}}
% \toprule
% Tool           & \#Examples \\ 
% \midrule
% W              & 115             \\ 
% P              & 105             \\ 
% R              & 103             \\ 
% NO             & 101             \\ 
% N              & 93              \\ 
% S              & 82              \\ 
% \bottomrule
% \end{tabular}
% \label{tab:source_generation_data_distribution}
% \end{table}

% \textbf{\#TODO: Table 2, Source Generation(SG) consists of 653 examples pertaining to the inclusion of H, but above definition is for 16 April dataset without H - small talk.}

% \begin{table}[h]
% \centering
% \caption{Summary of Datasets and Tasks}
% \begin{tabular}{@{}llr@{}} % Alignment of columns (left, left, right)
% \toprule
% Datasets                     & Task                             & \#Examples \\ 
% \midrule
% Source Generation (SG)       & Classification + Extraction      & 653        \\
% Intent Classification (IC)    & Classification                    & 4778       \\
% Product Identification (PI)   & Extraction                        & 867        \\
% Plan Generation (PG)          & Sequence Generation               & -          \\
% \bottomrule
% \end{tabular}
% \end{table}

% \subsection{Baselines}

% \roberta: 

% \ift:


 
% We use the following tasks and corresponding datasets to evaluate our model and the baselines: 

% \begin{itemize}
%     \item Retrieval Source Classification 
%     \item Retrieval Source Parameter Value Extraction 
%     \item Retrieval Source Plan Generation
% \end{itemize}

 
% \subsection{Experimental Setting} 


% \subsection{Experimental Results}

% \subsection{overall comparison with the baselines} 

% In this section, we compare the performance of REAPER with baselines. Table \ref{tab:overall_performance} shows the performance gain. Please refer to \url{/home/ubuntu/quic-efs/user/shrivagr/Projects/IFT_Eval/reaper_Eval/results/April26_24/classification_report_latex.txt} to get all the results.




% \subsubsection{Impact of IFT dataset} 

% \detokenize{model-ift_reaper_evolve_diverse_queries_3task_dynamic_incontext_v3}

% \detokenize{model-ift_reaper_nile_diverse_queries_3task_dynamic_incontext_v3}

\subsection{Ablation Study of Data Components}

We show the effectiveness of TEvo, DQS and IFT-Evolve in Table \ref{tab:reaper_ablation_study}. Apart from tool selection accuracy, we also investigate how these components help the model to follow instructions by introducing an adversarial prompt where we remove the \texttt{prod\_qna} tool and obtain REAPER predictions on the test dataset. Since the model is instructed to use only the specified tools it should not use \texttt{prod\_qna} to generate a plan. %We investigate recall of the \texttt{prod\_qna} tool based on the adversarial prompt. 
We measure instruction following capability \footnote{ We plan to evaluate performance on open IFT benchmarks, though we expect the performance to be similar to our domain specific evaluation} as (1-proportion of plans that use \texttt{prod\_qna}). 

%\begin{wraptable}{l}{\linewidth}
\begin{table}[b]
\centering
\caption{Impact of training data selection components}% \aj{add factoid adversarial recall}}
\label{tab:reaper_ablation_study}
\scriptsize
\begin{tabular}{@{}lrr@{}} % Alignment of columns (left, right, right)
\toprule
Model                    & Tool Accuracy   & Instruction Following \\ 
\midrule
REAPER       & 0.96  & 1.00\\
REAPER w/o \nileevolve    & 0.95 &  0.76\\
REAPER w/o \nileevolve\space and DQS   &     0.87 & 1.00\\
REAPER w/o \nileevolve, TEvo and DQS         &  0.91 & 0.85\\
\bottomrule
\end{tabular}
\end{table}
%\end{wraptable}


We observe that REAPER including all three components achieves both the highest tool selection accuracy and the best instruction following as none of its plans in the adversarial setting uses the omitted \texttt{prod\_qna} tool. 
%and a \texttt{prod_qna} recall is zero for the adversarial prompt as expected. Even though there are \texttt{prod_qna} data cases in our evaluation data, REAPER never predicts the class as it is strictly instructed to generate plan based on the given tools. 
When we remove \nileevolve\ data from training and use \nileift\ instead, tool selection accuracy drops. The model also loses instruction following capability as it uses \texttt{prod\_qna} in 24\% of plans. We observe the same phenomenon when we remove the TEvo (task diversity) and DQS (input query diversity) components from training, with a marked drop in accuracy when we drop DQS. This suggests that TEvo (task diversity) is needed for instruction following capabilities and DQS is needed for the model to understand the different query shapes. %When we remove DQS from the training pipeline and select a random set of queries, the model accuracy also drops. REAPER achieves the best balance between accuracy and instruction following ability overall. 




%\begin{wraptable}{r}{9cm}
% \begin{table}[tb]
% \centering
% \caption{Impact of training data selection components}% \aj{add factoid adversarial recall}}
% \label{tab:reaper_ablation_study}
% \tiny
% \begin{tabular}{@{}lrr@{}} % Alignment of columns (left, right, right)
% \toprule
% Model                    & Tool Accuracy   & Instruction Following \\ 
% \midrule
% REAPER       & 0.96  & 1.00\\
% REAPER w/o \nileevolve    & 0.95 &  0.76\\
% REAPER w/o \nileevolve\space and DQS   &     0.87 & 1.00\\
% REAPER w/o \nileevolve, TEvo and DQS         &  0.91 & 0.85\\
% \bottomrule
% \end{tabular}
% \end{table}
%\end{wraptable}




% \begin{table*}[b]
% \centering
% \caption{REAPER Data Proportion Study}
% \label{tab:data_proportion_study}
% \small
% \begin{tabular}{lccc} % Alignment of columns (left, left, right, right)
% \toprule
% Model & Accuracy & Tool-IFT Data Volume & IFT Data Volume \\
% \midrule
% REAPER + \nileevolve \space (40\%)+ TTG (3-task) & 0.93 & 19k & 60k \\
% REAPER + \nileevolve \space (50\%)+ TTG (3-task) & 0.93 & 19k & 75k \\
% REAPER + \nileevolve \space (60\%) + TTG (3-task)& 0.9 & 19k & 90k \\
% REAPER + \nileevolve \space (100\%) + TTG (3-task) & 0.86 & 19k & 147k \\
% REAPER + \nileevolve \space (100\%) + TTG (4-task) & 0.95 & 25k & 147k \\
% REAPER + \nileevolve \space (100\%) + TTG (5-task) & 0.94 & 32k & 147k \\
% \bottomrule
% \end{tabular}
% \end{table*}




 
% \begin{table}[h]
% \centering
% \caption{REAPER Ablation Study}
% \label{tab:reaper_ablation_study}
% \begin{tabular}{@{}llr@{}} % Alignment of columns (left, left, right)
% \toprule
% Model                    & Accuracy                             & Recall@Prod\_QnA \\ 
% \midrule
% REAPER       & 0.96     & 0.00       \\
% REAPER w/o \nileevolve    & 0.95                    &       0.24 \\
% REAPER w/o \nileevolve\space and DQS   &                  0.87       &    0.00   \\
% REAPER w/o \nileevolve, TEvo and DQS         &  0.91               & 0.15          \\
% \bottomrule
% \end{tabular}
% \end{table}

\subsection{Effect of Training Data Proportions }

Table \ref{tab:data_proportion_study} shows the different data proportions we experimented with in the training set.
We found that it is essential to either add ShareClaude (\nileift\ ) or its evolved version -- \nileevolve\ with REAPER plans in the training set. Without the generic data the model severely overfits to the REAPER use case and catastrophically forgets its instruction following capability. In this case, we see 77\% of queries hallucinate tools that the model has seen in training but are not in the instruction (IFT score = 0.23). %This helps the model to not  instruction following. 
On the flip side, with only generic-IFT training data, the model achieves only 20\% accuracy for the in-domain task of tool selection. 

The proportion of the generic IFT training data does affect the performance of the model. In the middle three rows of Table~\ref{tab:data_proportion_study}, we varied the proportion of the  \nileevolve\ data from 40\% to 60\%, while the last three rows show variation in the number of REAPER planning tasks (cf. Section~\ref{ssec:ttg}) per query. We see improvement in both metrics as we increase the amount of IFT data and REAPER plans up to a point, beyond which we see a drop in tool selection accuracy. We found the best balance between accuracy and instruction following is seen in a roughly 1:6 proportion of REAPER tasks and generic IFT (\nileevolve \space (100\%) + TTG (4-task)). However, we expect to tune these hyperparameters as we expand the system to new retrievers and use cases. 




%, and found that it is essential to use all of \nileevolve\ data. Then, we varied the number of tasks from the task generator from 3 to 5 which further increased the training data size and the proportion of the tool data. We found that as we add more tasks, the performance starts to degrade. We obtain the best performance with 100\% \nileevolve\ data and 4 tasks.



%We found that though skewing the training data to have a larger proportion REAPER-specific tasks, helps the accuracy, it significantly drops the instruction following capability of the model. However, beyond a point the model performance plateaus out on tool selection accuracy. The best balance between accuracy and instruction following is seen in a roughly 1:6 proportion of REAPER tasks and generic IFT (\nileevolve \space (100\%) + TTG (4-task)). %\aj{we need two extremes - 0\% IFT and 0\% TTG}

%With a general-purpose IFT dataset as a smoother, performance on planning task significantly degrades (up to 50\%). However, as general instruction following datasets are much better compared to \reaperift, we calibrated the data proportions by downsampling \nileevolve\ and upsampling \reaperift. 



\begin{table}[tb]
\centering
\caption{REAPER Data Proportion Study. Note that the REAPER tasks are generated using 6K unique in-domain queries, while the Generic IFT data is from open datasets.}%  \aj{need adversarial prod\_qna metrics. Otherwise the reviewer will question why IFT-Evolve(50\%) and TTG (4) is missing}}
\label{tab:data_proportion_study}
\scriptsize
%\begin{tabular}{lcccc} % Alignment of columns (left, left, right, right)
\begin{tabular}{lcccc} % Alignment of columns (left, left, right, right)
\toprule
Training data mix & Tool & \#REAPER & \#Generic & Instruction \\
 & Accuracy & tasks &  IFT & following \\
\midrule
\nileevolve \space (0\%)+ TTG (3-task) & 0.92 & 19k & 0k & 0.23\\
\nileevolve \space (100\%)+ TTG (0-task) & 0.2  & 0k & 147k & 0.71\\
\midrule
\nileevolve \space (40\%)+ TTG (3-task) & 0.93  & 19k & 60k & 1.00\\
\nileevolve \space (50\%)+ TTG (3-task) & 0.93 & 19k & 75k & 1.00\\
\nileevolve \space (60\%) + TTG (3-task)& 0.9  & 19k & 90k & 1.00\\
\midrule
\nileevolve \space (100\%) + TTG (3-task) & 0.86  & 19k & 147k & 1.00\\
\nileevolve \space (100\%) + TTG (4-task) & 0.95  & 25k & 147k & 1.00\\
\nileevolve \space (100\%) + TTG (5-task) & 0.94  & 32k & 147k & 1.00\\

\bottomrule
\end{tabular}
\end{table}

% As for each search query our data generation module TTG can generate several tasks, we increased the tasks from 3 to 5 and observed the change in accuracy.  
% We downsampled ift data and upsampled tool data to obtain a data balance as there is a prevalence of IFT data, but there is limited tool data. Table \ref{tab:data_proportion_study} shows the effect of both upsampling and downsampling.

% Downsampling the out-of-domain data alone while keeping the in-domain data constant does not seem to perform better on the accuracy compared to upsampling experiments. Thus, we chose to retain complete out-of-domain data so that the model can maintain its strong instruction-following capability, which is essential for tasks like keyword extraction that are not explicitly taught during the training process.



% \subsubsection{The effect of removing a tool from the prompt}

% We show how recall for the product question answering class drops as we remove the tool from the system prompt. We show that when using nile-evolve data as a smoother we get better instruction following. 




% \begin{table}[]
%     \centering
%     \begin{tabular}{lrrrr}
%     \toprule
%      & precision & recall & f1-score & support \\
%     \midrule
%     H & 0.91 & 0.91 & 0.91 & 54.00 \\
% N & 0.93 & 0.85 & 0.89 & 95.00 \\
% N O & 0.97 & 0.85 & 0.90 & 100.00 \\
% O & 0.00 & 0.00 & 0.00 & 0.00 \\
% P & 0.45 & 0.96 & 0.61 & 104.00 \\
% R & 0.00 & 0.00 & 0.00 & 105.00 \\
% S & 0.90 & 0.96 & 0.93 & 80.00 \\
% W & 0.93 & 0.90 & 0.92 & 115.00 \\
% accuracy & 0.76 & 0.76 & 0.76 & 0.76 \\
% macro avg & 0.63 & 0.68 & 0.64 & 653.00 \\
% weighted avg & 0.70 & 0.76 & 0.72 & 653.00 \\
% \bottomrule
    
%     \end{tabular}
%     \caption{REAPER classification results one product question answering tool is removed from the prompt. Reaper exactly follows instruction.}
%     \label{tab:my_label}
% \end{table}


% \paragraph{The effect on multi-step plan generation} with nile-evolve we can generate plan based on in context examples. 

% \subsubsection{How much of the evolved data is useful?} 

% \begin{tabular}{lrrrr}
% \toprule
%  & precision & recall & f1-score & support \\
% \midrule
% H & 0.00 & 0.00 & 0.00 & 0.00 \\
% N & 0.85 & 0.95 & 0.90 & 93.00 \\
% N O & 0.98 & 0.92 & 0.95 & 101.00 \\
% P & 0.93 & 0.93 & 0.93 & 105.00 \\
% R & 0.90 & 0.99 & 0.94 & 103.00 \\
% S & 1.00 & 0.91 & 0.96 & 82.00 \\
% W & 0.95 & 0.88 & 0.91 & 115.00 \\
% accuracy & 0.93 & 0.93 & 0.93 & 0.93 \\
% macro avg & 0.80 & 0.80 & 0.80 & 599.00 \\
% weighted avg & 0.94 & 0.93 & 0.93 & 599.00 \\
% \bottomrule
% \end{tabular}

% \detokenize{model-reaper_evolve_downsample_50}

% \begin{tabular}{lrrrr}
% \toprule
%  & precision & recall & f1-score & support \\
% \midrule
% H & 0.00 & 0.00 & 0.00 & 0.00 \\
% N & 0.95 & 0.86 & 0.90 & 93.00 \\
% N O & 0.92 & 0.96 & 0.94 & 101.00 \\
% P & 0.93 & 0.91 & 0.92 & 105.00 \\
% R & 0.91 & 0.98 & 0.94 & 103.00 \\
% S & 0.99 & 0.90 & 0.94 & 82.00 \\
% W & 0.92 & 0.94 & 0.93 & 115.00 \\
% accuracy & 0.93 & 0.93 & 0.93 & 0.93 \\
% macro avg & 0.80 & 0.79 & 0.80 & 599.00 \\
% weighted avg & 0.93 & 0.93 & 0.93 & 599.00 \\
% \bottomrule
% \end{tabular}

% \detokenize{model-reaper_evolve_downsample_60}

% \begin{tabular}{lrrrr}
% \toprule
%  & precision & recall & f1-score & support \\
% \midrule
% H & 0.00 & 0.00 & 0.00 & 0.00 \\
% N & 0.95 & 0.77 & 0.85 & 93.00 \\
% N O & 0.89 & 0.95 & 0.92 & 101.00 \\
% P & 0.79 & 0.96 & 0.87 & 105.00 \\
% R & 0.97 & 0.90 & 0.93 & 103.00 \\
% S & 0.91 & 0.95 & 0.93 & 82.00 \\
% W & 0.95 & 0.84 & 0.89 & 115.00 \\
% accuracy & 0.90 & 0.90 & 0.90 & 0.90 \\
% macro avg & 0.78 & 0.77 & 0.77 & 599.00 \\
% weighted avg & 0.91 & 0.90 & 0.90 & 599.00 \\
% \bottomrule
% \end{tabular}




% \subsubsection{How many tasks are useful to be generated from the task generator?}

% Upsampling the in-domain data while retaining the complete out-of-domain data leads to a significant improvement in source classification task accuracy. This suggests that increasing the ratio of in-domain to out-of-domain data (1:5.8) can positively impact the model's performance on the target task of source classification. 



% \subsubsection{How helpful is are the diverse set of queries?} 

% \detokenize{ift_reaper_mistralinstructv2_sc_3kds_1xtool_smalltalk_3task_cleaned}

% \detokenize{model-ift_reaper_nile_ift_diverse_queries_3task_dynamic_incontext_v3}



% \subsubsection{Can we use a new tool without any training?} 


% \subsection{Parameter Extraction:} 

% As REAPER achieves 96\% accuracy in identifying the right tools, we use the queries identified by REAPER as product search and order history for evaluating the capability of REAPER in extracting product names and date time. When the intent of a search query is related to product search, REAPER uses the \texttt{product\_search} tool and identifies search query terms from a natural language query. 


\subsection{Analysis on Generalization}

%\begin{wrapfigure}{r}{0.66\textwidth}
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.99\linewidth]{New_Complex_Plans_Updated.png}
    \caption{Plans for new use cases. The first plan hallucinates the product\_id but the second plan shows no hallucinations after we add just 25 post-purchase examples to training set}\label{fig:novel_multi_step}
\end{figure}
%\end{wrapfigure}

\paragraph{Can REAPER generate a novel plan?} Our training data has multi-step plans only in the order status context. Even so, using in-context examples alone REAPER is able to generate the right tools sequences for use-cases for query shapes it has never seen before. We did see occasional hallucinations. We added only 25 more diverse multi-step examples and REAPER was able to generate accurate brand new plans without hallucinations. Figure ~\ref{fig:novel_multi_step} shows some examples. 
%REAPER can generate a novel plans that it has never seen during training based on in-context examples alone. For the query \textit{Is my desk made of real wood} as an example which clearly requires more than one retrieval tool as well as a multi-step response. The model was not trained with such multi-step plans and we were able to generate a reasonable plan by simply adding a relevant in-context example. REAPER generated the following plan:



%Please refer to the slack post for details: \url{https://amzn-wwc.slack.com/archives/C06JU9HLR2N/p1714028179717779}

\paragraph{Can REAPER be fine-tuned with limited data?} 



% \begin{table}[!htpb]
% \caption{Comparison of REAPER performance with Baselines on Human Small Talk Class}
% \label{tab:human_small_talk}

% \begin{tabular}{|l|lll|llll|}
% \hline
%                                & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}Mistral\\ (No fine-tuning)\end{tabular}}                                                                                                   & \multicolumn{4}{l|}{Reaper}                                                                                                                   \\ \hline
% Classes                        & \multicolumn{1}{l|}{P}             & \multicolumn{1}{l|}{R}             & F1             & \multicolumn{1}{l|}{P}   & \multicolumn{1}{l|}{R}   & \multicolumn{1}{l|}{F1} & \begin{tabular}[c]{@{}l@{}}\#Training\\ Examples\end{tabular} \\ \hline
% Human Small Talk               & \multicolumn{1}{l|}{91}            & \multicolumn{1}{l|}{72}            & 80                                                                  & \multicolumn{1}{l|}{94}  & \multicolumn{1}{l|}{91}  & \multicolumn{1}{l|}{92} & \multicolumn{1}{c|}{286}     

% \\ \hline
%                       \end{tabular}
%\end{table}

% \begin{table}[!htpb]
% \caption{Comparison of REAPER performance with Baselines on Human Small Talk Class}
% \label{tab:human_small_talk}

% \begin{tabular}{|l|lll|llll|llll|}
% \hline
%                                & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}Mistral\\ (No fine-tuning)\end{tabular}} & \multicolumn{4}{l|}{Production Classifier}                                                                                                   & \multicolumn{4}{l|}{Reaper}                                                                                                                   \\ \hline
% Classes                        & \multicolumn{1}{l|}{P}             & \multicolumn{1}{l|}{R}             & F1            & \multicolumn{1}{l|}{P}  & \multicolumn{1}{l|}{R}   & \multicolumn{1}{l|}{F1} & \begin{tabular}[c]{@{}l@{}}\#Training\\ Examples\end{tabular} & \multicolumn{1}{l|}{P}   & \multicolumn{1}{l|}{R}   & \multicolumn{1}{l|}{F1} & \begin{tabular}[c]{@{}l@{}}\#Training\\ Examples\end{tabular} \\ \hline
% Human Small Talk               & \multicolumn{1}{l|}{91}            & \multicolumn{1}{l|}{72}            & 80            & \multicolumn{1}{l|}{-}  & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}  & \multicolumn{1}{c|}{-}                                                              & \multicolumn{1}{l|}{94}  & \multicolumn{1}{l|}{91}  & \multicolumn{1}{l|}{92} & \multicolumn{1}{c|}{286}     

% \\ \hline
%                       \end{tabular}
% \end{table}


A practical use-case of REAPER is adapting to a new retrieval source with limited amount of data. We tested this, by adding a new \texttt{no-evidence} class called \texttt{human\_small\_talk}. We added only 286 examples of this class to our training data and saw that the model achieves an F1 score of 0.92 which comparable performance to other sources trained with order of magnitude more data. 

%\begin{wrapfigure}{r}{0.66\textwidth}
%\end{wrapfigure}

\begin{figure}[tb]
%\label{fig:novel_tool}
    \centering
    \includegraphics[width=0.9\linewidth]{Novel_Tools_Updated.png}
    \caption{REAPER plans with tools not in training data}
     \label{fig:novel_tool}
\end{figure}

\paragraph{Can REAPER use a novel tool?}

We explore how well REAPER can learn to use a new tool without any training data at all and based solely on in-context examples for the tool. To do this, we added a new toolcalled \texttt{compatible\_products} with its description and a few demonstrative examples in the prompt and found that REAPER is able to generate a valid plan. For the query \textit{ink cartridge for HP 4650}, REAPER generated the plan in Figure~\ref{fig:novel_tool}. This also shows that REAPER has maintained its instruction following ability. 



%\paragraph{Can REAPER generalize to a different distribution?} Shoppability keyword extraction slack post: \url{https://amzn-wwc.slack.com/archives/C06JU9HLR2N/p1714583520448509}

% \subsubsection{Source selection}
% \subsubsection{Source order}
% \subsubsection{Argument Rouge-L}

% \subsection{Capabilities}
% \subsubsection{Plan accuracy}
% \subsubsection{Ease of adding new source}
% \subsubsection{Extending to new tasks}


==> _old/07-27-2024/methodology.tex <==
\section{REAPER} 

To develop an LLM that meets the requirements of Section~\ref{sec:prob-statement}, we need a reasonably small LLM with strong instruction following abilities. We use \ift ~\cite{jiang2023mistral} based on its performance on open IFT benchmarks. However, even with significant prompt tuning and in-context examples, the Mistral model was prone to hallucinations (see Figure~\ref{fig:mistral-plans-1} for examples). Hence, we fine-tune the model for our use case. In this section, we explain our methodology for designing the REAPER prompt and selecting fine-tuning data to maintain instruction following and eliminate hallucinations while learning the specialized task of retrieval tool planning. % so that the model does not hallucinate but still is able to maintain instruction following capabilities in the retrieval planning context. 

\begin{figure}[tb]
%\label{fig:Mistral-plans}
    \centering
    \includegraphics[width=\linewidth]{Mistral_Plan_Generation_1.png}
    % \caption{Example: Mistral plans }
    %\label{fig:mistral-plans-1}
%\end{figure}
% \end{wrapfigure}

% \begin{wrapfigure}{r}{0.66\textwidth}
%\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Mistral_Multi_Step_Plan_Generation_2.png}
    \caption{Example: Mistral plans. For simple queries (first and third query) Mistral produces the right plans. However, for multi-step retrieval Mistral goes beyond just retrieval evidence generation, hallucinating steps like Compare (second plan) and Extract estimated delivery time (fourth plan).}
    \label{fig:mistral-plans-1}
\end{figure}


%Our goal is to develop a fine-tuned LLM model that can generate a retrieval plan for a customer question -- in the context of a conversation -- using the tools available to it. Figure~\ref{fig:reaper-plans} shows a few examples of plans generated by the REAPER model. The plans can be a single retrieval source (single-step plan) or multi-step retrieval plan requiring CoT reasoning. However, we expect the model to retain its ability to follow instructions as we want the model to be able to use novel tools and solve query understanding tasks that are not specified using tools. To this end, we aim to achieve a balance between general instruction following (e.g., write a poem), query understanding (e.g., identify the target product from a conversation and generate keywords to retrieve it), and tool-instruction following (e.g., use the following tools to summarize today's weather). In order to achieve this balance, we combine several annotated data sources and apply a number of techniques so that the model does not overfit on a particular type of instruction. 



\subsection{REAPER Prompt Design}
\label{sec:reaper_prompt}
%The instruction fine-tuning data for a generative large language model is a set of $n$ pairs, $T = {\{(p_k, y_k)}\}_{k=1}^{n}$, where $p_k$ is a prompt and $y_k = (f_1^k(a_1), f_2^k(a_2), \ldots, f_l^k(a_l))$ is the output plan which is a sequence of tools with their parameters. For clarity, we will drop the suffix $k$, with the understanding that the following is applied to the $n$ fine-tuning data points. An example prompt is shown in Appendix~\ref{app_reaper_prompt}

An LLM prompt $p$ consists of an input $x$, an instruction set $I$, and a set of $m$ in-context examples, $E = {\{(\Tilde{x}_1, \Tilde{y}_1), (\Tilde{x}_2, \Tilde{y}_2), \ldots, (\Tilde{x}_m, \Tilde{y}_m)\}}$ that help the model understand the desired task. 

In our prompt, $I$ includes instructions like the role of the LLM as well as all the tools $T = \{\Tilde{f}_1, \Tilde{f}_2, \ldots, \Tilde{f}_t\}$. The tools are essentially API calls that the REAPER LLM needs to understand. We provide the tool name, tool signature, its natural language description and an example usage in the prompt. Finally, $I$ contains task instructions and constraints. Exemplar elements of the prompt are shown here: % (refer Appendix~\ref{app_reaper_prompt} for exact prompt)%eg: \texttt{only use the tools specified above}) 


\begin{minted}[breaklines=true, showspaces=False, frame=lines, breaksymbol=, fontfamily=zi4, fontsize=\footnotesize]{text}

### Role:
You are an AI assistant to a salesperson at a big retail store. Your goal is to find the right information to help the salesperson answer the customer's question. 

### System Instruction:
Your goal is to generate a step by step plan using the tools listed below to get the information needed to answer a customer question. The output of one tool can be fed to another in a sequential manner. Each step may use only one tool. Some parameters of a tool can be generated with help of provided capabilites.

The set of the candidate tools, their definitions, example usages are:

1. prod_qna - Tool: Fetches specific information for a particular aspect or attribute of the product . It needs a product ID and a query as input. 
...
\end{minted}

% As input, you are provided a context and customer question. The context is 
% either empty or provides you information from where the customer is 
% interacting with the salesperson, i.e page type or or provides you 
% information about the product page from where the customer is 
% interacting with the salesperson, i.e product title and product ID.

% The set of the candidate tools, their definitions, example usages are:

% 1. prod_qna - Tool: Fetches specific information for a particular aspect or attribute of the product . It needs a product ID and a query as input. 



%, and a set of natural language instructions, $S_k$ providing the directions and constraints on how to use the tool set $T_k$ to obtain retrieval evidences. Each tool $\Tilde{f}_1^k \in I_k$ in the prompt is provided with a function signature describing its name, description, and usage of its arguments. 


%In combination, $I_k$ and $E_k$ directs and provides demonstrations to the LLM to understand the task and process the input and accordingly generate the desired output. It is often required to construct a structured and complex prompt to generate the target output. 

For our case, the input $x = \{q, c\}$ includes the customer query, $q$ and page context, $c$. A customer can reference information gathered during their shopping journey. So on a product Detail Page (DP), we include the product title in $c$. On non-product pages, like Search Results Page, Landing Page, Cart, etc., $c$ is empty. Page context is necessary for anaphoric and contextual de-referencing. For example, when a customer asks \textit{"What is your favorite color"} on the general Amazon.com page, they are simply engaging in small talk with Rufus. However, if they ask the same question on the DP of say a t-shirt that is available in multiple colors, they expect Rufus to respond in the context of that t-shirt. In former (small-talk) case, Rufus may wish to answer with no evidence along the lines of \textit{"I am an AI assistant and do not have favorite colors"} (paraphrased for brevity). In the latter case, Rufus will use evidence from reviews to deduce the popular colors or sentiment around different colors to form an answer. 

% Below we show some exemplar components of the prompt. The actual prompt is shown in Appendix~\ref{app_reaper_prompt}

% \begin{itemize}
%     \item $I$: Your goal or task is to generate a step by step plan using the tools listed below to get the information needed to answer a customer question. 
%     \item $f_1 \in T_k:$ prod\_qna - Tool: Fetches specific information for a particular aspect or attribute of the product. It utilizes product ID and product title provided as input.  
%     \item $\Tilde{x}_1 \in E$: \{$c$ = "product\_id": "B09GW671M2", "product\_title": "Brenna 4 Pack Large Food Storage Containers", $q$ = "Is the lid airtight?" \}
%     \item $\Tilde{y}_1 \in E$: Step 1: \#E1 = prod\_qna("B09GW671M2", "Is the lid of Brenna 4-Pack Large Food Storage Containers airtight?")  
% \end{itemize}


%$I_k$ include system instructions like, the Role the LLM is expected to play and the descriptions and example usage of the different tools available to the LLM. $I_k$ also includes task instructions that tell the LLM how to process the input and what we expect in the output. Finally, we can also include a set of $m$ in-context examples in the prompt. An example prompt for REAPER is shown in Appendix~\ref{app_reaper_prompt}


\subsection {REAPER Data Generation Approach}

For REAPER we aim to balance two contrasting objectives: 1) the model needs to generate the plan for an in-domain task in a precise format with the right tool signatures, 2) the model should be able to understand changes in the input including nuanced changes in instructions and tools and adapt the plans accordingly. We can meet the first requirement by training the model with a large number of precise REAPER plans. However, this causes the model to overfit on the planning task and it loses its instruction following and reasoning capability. On the flip side, without enough plans in the training data, we see that the model tends to hallucinate responses. %We  %Our situation is further complicated since we want to train the model primarily for the planning task - which means that the model needs to work with a single prompt.   

%In order to achieve a balance between both requirements, we start with a strong base model that has good instruction following capabilities and train it further. For our purpose we chose the \textbf{Mistral-Instruct-v0.2} public checkpoint available via HuggingFace. \aj{I just put this in the intro to hte section :)}

An important design consideration for fine-tuning an LLM for instruction following is to provide it with a diverse set of prompt and output pairs so that it does not overfit on a specific task template and catastrophically forget its ability to closely follow instructions. This becomes particularly challenging since our primary task is retrieval planning and so the scope of %when we have several training data examples for a target task where the scope of 
introducing diversity in the instruction set is limited. We develop the following modules for different aspects of input and output data diversity. 

\subsubsection{Tool Evolve (TEvo): Evolution of Base Tool Prompt}We introduce a novel module  \textbf{Tool Evolve (TEvo)} that takes the tool prompt as input and produces a semantically similar prompt in a way that the output, $y$ does not change. The technique is similar to introducing adversarial noise into images for building robust image classifiers \cite{10.1145/3485133}. To force our model to pay attention to tools and their corresponding descriptions, we select the tool(s) required to for a particular query and a random subset of the remaining tools to include in the instruction section of our prompt. We also create a pool of name variation and description paraphrases for each tool and sample from these. For example, to answer questions about a product, our tool names can be \texttt{prod\_qna}, \texttt{product\_information}, \texttt{product\_facts}, etc. Finally, we also vary in-context examples by sampling from a small pool of human generated plans.



%Section \ref{sec:reaper_prompt} introduces our prompt template for creating tool-usage training data. 
%As our human-annotated training data contains eight tools, to create prompt diversity, we randomly select $t$ tools from $T_k$ that do not appear in output plan, and remove them from $p_k$. We also paraphrase the names and descriptions of each the $t$ selected tools. We create a pool of paraphrases for tool names and descriptions of the eight tools in our training data and randomly select paraphrases for the $t$ tools to construct a training example. An example paraphrase of the tool \texttt{prod\_qna} introduced in section \ref{sec:reaper_prompt} is \texttt{product\_question\_and\_answer}. Furthermore, we vary the $m$ in-context examples, $E_k$, by selecting them randomly from a small pool (20 examples per tool) of examples that is separate from the training data. 

%While TEvo creates adversarial input, we also employ another module to create diversity in output $y_k$ \sn{what is the other module? Sounds confusing here @sheikh}. This is because the output of supervised tool-usage data is a sequence of tools along with their parameters and values, and fine-tuning an LLM on such data could make it respond to any instruction in tool format. 

\subsubsection{Tool-Task Generator (TTG)}
\label{ssec:ttg}
%To avoid overfitting to a specific output format, we create a diverse set of tasks from the supervised tool-usage data $T$. 
In Wizardlm~\cite{xu2023wizardlm}, the authors increase the complexity of simple tasks and add these tasks to the IFT training data in order to improve the instruction following capability of an LLM.  Similarly, we introduce an approach to create diversified tasks related to retrieval planning. This forces the LLM to understand tools and retrieval plans. 

%We introduce a novel module \textbf{Tool-Task Generator (TTG)}, that creates a number of tasks from a $(p_k, y_k)$ pair.

Given a primary task of generating a retrieval plan $T_{prim} = (\mathbf{x}, \mathbf{y})$, where $\mathbf{x}$ is the input containing the query $q$ and context $c$, we transform the task into multiple related tasks. % $T_i = f_i(T_{prim})$.  

%Let the primary  task be the generation of a retrieval plan $\mathbf{y}$ given a customer query along with context $\mathbf{x}$ . We denote this primary task as $T_\text{primary} = (\mathbf{x}, \mathbf{y})$.

%To diversify the training and enhance the model's generalization, we introduce a set of $K$ secondary tasks $\{T_1, T_2, \dots, T_K\}$. Each secondary task $T_i$ is defined as a transformation of the primary task $T_\text{primary}$, such that:

\begin{equation}
    T_i = f_i(T_\text{primary})
\end{equation}

where $f_i$ is the task-specific transformation function. The secondary tasks are target specific capabilities like: 

\begin{enumerate}
    \item Generate query from a plan: $T_1 = \text{generate\_query}(\mathbf{y})$, 
    \item Complete partial plan: $T_2 = \text{complete\_partial\_plan}(\mathbf{x}, \mathbf{y}_\text{partial})$, 
    \item Identify the right tools: $T_3 = \text{identify\_tools}(\mathbf{x})$, 
    \item Masked step completion: 
    
    $T_4 = \text{complete\_masked\_step}(\mathbf{x}, \mathbf{y}_\text{masked})$, 
    \item Reordering steps in coorect sequence: 
    
    $T_5 = \text{reorder\_steps}(\mathbf{x}, \mathbf{y}_\text{shuffled})$, 
    \item Masked parameter identification: 
    
    $T_6 = \text{identify\_masked\_params}(\mathbf{x}, \mathbf{y}_\text{masked})$, 
    \item Limit tools in plan to only the ones specified in the prompt: 
    
    $T_7 = \text{use\_provided\_tools}(\mathbf{x}, \text{tools})$ \# This will %\aj{Need an intuitive descriptor for this}
\end{enumerate}
The TTG module creates diverse task-target pairs $\{(\mathbf{p}_1, \mathbf{y}_1), %(\mathbf{p}_2, \mathbf{y}_2), 
\dots, \newline(\mathbf{p}_N, \mathbf{y}_N)\}$ by applying the secondary task transformations $f_i$ to the primary task $T_\text{primary}$. We then sample from this diverse set of tasks to fine-tune the REAPER model, with the aim of developing a robust understanding of the overall task structure and enhancing its ability to generate retrieval plans for complex customer queries.

\subsubsection{Diverse Query Sampler (DQS)}
In addition to adding diversity in prompt using TEvo and diversity in output using TTG, we also diversify the input $x_k$, which is a question from a customer with a page context. Similar queries cause the model to fixate on particular query shapes leading to performance degradation when the model encounters out-of-distribution cases. To this end, we propose \textbf{Diverse Query Sampler (DQS)} that automatically generates a sample of customer queries that are semantically dissimilar. We annotate the diverse samples with relevant tools and parameters based on the conversational context. 

%Recall that the primary task $T$ was defined as generating a retrieval plan $y$ given a customer query $\mathbf{x}$ and context. The DQS module aims to introduce diversity in the input $\mathbf{x}$, which is the customer query. 
Given a high-quality curated initial (small) pool of customer queries, $\mathbf{Q}_\text{initial} = \{\mathbf{x}_1, \mathbf{x}_2, ..., \mathbf{x}_N\}$ and a larger pool of generated or sampled customer queries $\mathbf{Q}_\text{large}$, DQS introduces diversity by:

1. Generating BERT-based embeddings $\mathbf{e}_i$ for each query $\mathbf{x}_i$ in $\mathbf{Q}_\text{large}$, where $\mathbf{e}_i = \text{RoBERTa}(\mathbf{x}_i)$.

2. Calculating the pairwise cosine similarity between the query embeddings in $\mathbf{Q}_\text{initial}$ and $\mathbf{Q}_\text{large}$ to obtain a similarity matrix $\mathbf{S}$, where $\mathbf{S}[i,j] = \cos(\mathbf{e}_i, \mathbf{e}_j)$ for $\mathbf{x}_i \in \mathbf{Q}_\text{initial}$ and $\mathbf{x}_j \in \mathbf{Q}_\text{large}$.

3. Identifying the most similar and most dissimilar pairs of queries in $\mathbf{Q}_\text{large}$ based on the similarity matrix $\mathbf{S}$. Let these be the set of queries at the extremes of diversity, denoted as $\mathbf{Q}_\text{extreme}$.

4. Removing $\mathbf{Q}_\text{extreme}$ from $\mathbf{Q}_\text{large}$ to obtain a refined pool $\mathbf{Q}_\text{refined} = \mathbf{Q}_\text{large} \setminus \mathbf{Q}_\text{extreme}$.

5. Randomly sampling a subset of queries from the larger pool $\mathbf{Q}_\text{large}$ to obtain the final diverse set of customer queries $\mathbf{Q}_\text{diverse}$. The size of $\mathbf{Q}_\text{diverse}$ is chosen such that $|\mathbf{Q}_\text{diverse}| = |\mathbf{Q}_\text{initial}|$.

The goal of this process is to ensure that the queries in $\mathbf{Q}_\text{diverse}$ have a balanced representation of semantic diversity, reducing model bias and enhancing the ability of REAPER to generalize across different customer information needs.

%example pool create prompt variation by randomly selecting  from a pool to con


%An Instruction Fine-Tuned (IFT) LLM is generally able solve any arbitrary task when properly instructed using prompts. However, we found that relatively smaller LLMs (e.g., Mistral-7B-Instruct-v0.2) that are less expensive to deploy often fail to follow complex tool-usage instructions and thus hallucinate in the output. As a remedy to this phenomenon, we propose to fine-tune an LLM with tool-usage training data -- created using our prompt template introduced in \ref{sec:reaper_prompt} -- to enable it to effectively use tools to retrieve evidence for query planning. However, it often leads to overfitting when an LLM is fine-tuned with task specific data. In this section, we describe how we created prompt variations to control overfitting. 

% In section \ref{sec:reaper_prompt}, we proposed a prompt design template with required notation. Here, we provide an example of each of the prompt component. 




% that includes an instruction set ($I_k$), in-context examples($E_k$), natural language customer question  along with context ($x_k$), and a retrieval plan ($y_k$). Our training data is human labeled -- meaning that a human judge provided the query plan $y_k$ given $x_k$.  



% prompt template that includes the components to construct instructions for fine-tuning an LLM to enable it to use tools In section \ref{sec:reaper_prompt} we introduced the prompt  several components of the prompt that we use for training. Instruction Set ($I_k$): We provide a task description for tool usage to REAPER in a way that we would provide it to a human annotator. In the instruction set we specify that there will be a list of tools along with their parameter descriptions and REAPER will have to use those tools in the correct sequence with the correct parameters to retrieve evidence associated with a customer information need, $x_k$. We also provide instructions to constrain REAPER output using instruction prefixes such as "(VERY IMPORTANT!!)". A detailed description of $I_k$ is provided in the Appendix section. 

%\paragraph{Tool List:} The task description, $I_k$ includes a list of tools along with their name

%\paragraph{In-Context Examples of Tool Usage:} 





%TODO: Describe the base prompt and show diversification results based on an example. This can also go into the intro. 
%set of instructions, input, and output pairs so that it generalizes to an unseen task and produce novel output that solves the task. 


%to help the LLM to understand the task and process the input accordingly to produce the desired output $o_i$.  and   The prompt can be simple or complex depending on the complexity of the task. This work focuses on complex prompts where 


%$$ has the format of prompt ($p$), output pairs where  training data The training data for the fine-tuning process 


%In order to achieve this balance, we 


%We aim to achieve this balance by combining a general instruction following dataset and a tool-usage dataset. 





% Generally, a prompt is constituted from an instruction, $i$, and an input, $x$. For example, for the task of keyphrase extraction   

% A prompt has three parts: instruction, input, and output. 

% We design three components to construct an instruction set for fine-tuning a pre-trained LLM: Query Sampler, Task Sampler and  

\subsubsection{General purpose IFT data}
To retain the model's instruction following ability, we include general purpose instruction fine-tuning datasets in addition to the REAPER tool planning data. We use ShareClaude and open-source tool usage data from ToolAlpaca \cite{tang2023toolalpaca} for generic IFT data. We call this dataset \nileift\ . To further enhance the model's ability to follow nuanced changes in the input instruction, we utilize a framework inspired from Evol-Instruct \cite{xu2023wizardlm} that automatically generates more complex IFT data by adding constraints on simple instructions and samples to maintain a roughly equal proportion of query complexity as measured by the prompt length used for the task. We call this dataset \nileevolve. Our final fine-tuning dataset, \reaperift\ is a combination \nileift/\nileevolve\ and our tool-annotated queries which are diversified using TEvo, TTG and DQS. 

%This is a confidential dataset available internally to the Rufus team and consists of 150K general purpose IF tasks with varying levels of complexity. 

%\vspace{1cm}


% \subsection{Training Pipeline}
% We train the REAPER model on a cluster of 4 AWS p4d.24xlarge instances using AWS Batch, which took approximately 20 hours to complete. We used Fully Sharded Data Parallelism (FSDP) to enable efficient distributed training across the 4 GPU-equipped instances. FSDP partitions the model parameters across the available devices, reducing the memory footprint on each GPU and allowing for faster convergence. We also Incorporated gradient checkpointing to further optimize the training efficiency. This distributed training approach using FSDP allowed the REAPER model to be efficiently trained in reasonable time.

